Experimental Investigation of the Inelastic Response of Pig and Rat Skin under Uniaxial Cyclic Mechanical Loading

Skin is a highly non-linear, anisotropic, rate dependent inelastic, and nearly incompressible material which exhibits substantial hysteresis even under very slow (quasistatic) loading conditions. In this paper, a series of uniaxial cyclic loading tests of porcine and rat skin at different strain rates and with samples oriented in different directions (with respect to the spine) were conducted to study the effect of strain rate and samples orientations with respect to spine on mullins effect and skin inelastic response. A noteworthy feature of skin is that, similar to certain filled rubbers, its mechanical response shifts after the first extension and exhibits softening and hysteresis when loaded under cyclic tension and mullins effect is observed. The results of these strain-controlled cyclic loading tests also indicated that the extent of softening is different for different strain rates and orientations. Also a substantial hysteresis persists even at very low strain rates indicating inelastic behavior beyond the rate sensitive viscoelastic response. Through this series of experiments, by investigating the effect of strain rate on pig skin and rat skin, we conclude that the skin response is rate dependent but inelastic and shows irreversible changes in fiber orientation which are observed in histology results. Also, skin shows persistent deformation that is only partially recovered even after a long period of unloading.

==> Experimental Investigation of the Inelastic Response of Pig and Rat Skin under Uniaxial Cyclic Mechanical Loading/reference.tex <==

@article{Mullins48,
title = {Effect of Stretching on the Properties of Rubber},
journal = {Rubber Chemistry and Technology},
volume = {21},
number = {2},
pages = {281-300},
year = {1948},
doi = {10.5254/1.3546914},
URL = {http://dx.doi.org/10.5254/1.3546914   },
eprint = { http://dx.doi.org/10.5254/1.3546914  }
}

@inbook{McGrath10,
author = {J. A. McGrath and J. Uitto},
publisher = {Wiley-Blackwell},
isbn = {9781444317633},
title = {Anatomy and Organization of Human Skin},
booktitle = {Rook's Textbook of Dermatology},
chapter = {3},
pages = {1-53},
doi = {10.1002/9781444317633.ch3},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/9781444317633.ch3},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/9781444317633.ch3},
year = {2010},
}


@article{Naylor11,
title = "Molecular aspects of skin ageing ",
journal = "Maturitas ",
volume = "69",
number = "3",
pages = "249 - 256",
year = "2011",
note = "",
issn = "0378-5122",
doi = "http://dx.doi.org/10.1016/j.maturitas.2011.04.011",
url = "http://www.sciencedirect.com/science/article/pii/S0378512211001496",
author = "Elizabeth C. Naylor and Rachel E.B. Watson and Michael J. Sherratt",
}

@article{Minns73,
title = "The role of the fibrous components and ground substance in the mechanical properties of biological tissues: A preliminary investigation ",
journal = "Journal of Biomechanics ",
volume = "6",
number = "2",
pages = "153 - 165",
year = "1973",
note = "",
issn = "0021-9290",
doi = "http://dx.doi.org/10.1016/0021-9290(73)90084-5",
url = "http://www.sciencedirect.com/science/article/pii/0021929073900845",
author = "R.J. Minns and P.D. Soden and D.S. Jackson"
}

@article{Brown73,
title={A scanning electron microscope study of the effects of uniaxial tension on human skin},
author={Brown, Ian A},
journal={British Journal of Dermatology},
volume={89},
number={4},
pages={383--393},
year={1973},
publisher={Wiley Online Library}
}

@Inbook{Xu11,
author="Xu, Feng
and Lu, Tianjian",
title="Skin Mechanical Behaviour",
bookTitle="Introduction to Skin Biothermomechanics and Thermal Pain",
year="2011",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
chapter="5",
pages="87-104",
isbn="978-3-642-13202-5",
doi="10.1007/978-3-642-13202-5_5",
url="https://doi.org/10.1007/978-3-642-13202-5_5"
}


@article{OXLUND88,
title = "The role of elastin in the mechanical properties of skin",
journal = "Journal of Biomechanics",
volume = "21",
number = "3",
pages = "213 - 218",
year = "1988",
note = "",
issn = "0021-9290",
doi = "http://dx.doi.org/10.1016/0021-9290(88)90172-8",
url = "http://www.sciencedirect.com/science/article/pii/0021929088901728",
author = "Hans Oxlund and Jan Manschot and A. Viidik",
}


@article{Diani09,
  title={A review on the Mullins effect},
  author={Diani, Julie and Fayolle, Bruno and Gilormini, Pierre},
  journal={European Polymer Journal},
  volume={45},
  number={3},
  pages={601--612},
  year={2009},
  publisher={Elsevier}
}

@article{lion96,
  title={A constitutive model for carbon black filled rubber: experimental investigations and mathematical representation},
  author={Lion, Alexander},
  journal={Continuum Mechanics and Thermodynamics},
  volume={8},
  number={3},
  pages={153--169},
  year={1996},
  publisher={Springer}
}


@article{Treloar44,
author = { L. R. G.   Treloar },
title = {The Elasticity of a Network of Long-Chain Molecules. II},
journal = {Rubber Chemistry and Technology},
volume = {17},
number = {2},
pages = {296-302},
year = {1944},
doi = {10.5254/1.3546653},
URL = {http://dx.doi.org/10.5254/1.3546653},
eprint = { http://dx.doi.org/10.5254/1.3546653}
}


@article{Simo87,
title = "On a fully three-dimensional finite-strain viscoelastic damage model: Formulation and computational aspects",
journal = "Computer Methods in Applied Mechanics and Engineering",
volume = "60",
number = "2",
pages = "153 - 173",
year = "1987",
note = "",
issn = "0045-7825",
doi = "http://dx.doi.org/10.1016/0045-7825(87)90107-1",
url = "http://www.sciencedirect.com/science/article/pii/0045782587901071",
author = "J.C. Simo",
}

@article{miehe95,
  title={Discontinuous and continuous damage evolution in Ogden-type large-strain elastic materials},
  author={Miehe, Ch},
  journal={European journal of mechanics. A. Solids},
  volume={14},
  number={5},
  pages={697--720},
  year={1995},
  publisher={Elsevier}
}
@article{Guth43,
author = {Hubert M. James and Eugene Guth},
title = {Theory of the Elastic Properties of Rubber},
journal = {The Journal of Chemical Physics},
volume = {11},
number = {10},
pages = {455-481},
year = {1943},
doi = {10.1063/1.1723785},
}

@article{Arruda93,
title = "A three-dimensional constitutive model for the large stretch behavior of rubber elastic materials",
journal = "Journal of the Mechanics and Physics of Solids",
volume = "41",
number = "2",
pages = "389 - 412",
year = "1993",
note = "",
issn = "0022-5096",
doi = "http://dx.doi.org/10.1016/0022-5096(93)90013-6",
url = "http://www.sciencedirect.com/science/article/pii/0022509693900136",
author = "Ellen M. Arruda and Mary C. Boyce",
}

@article{Govindjee91,
title = "A micro-mechanically based continuum damage model for carbon black-filled rubbers incorporating Mullins' effect",
journal = "Journal of the Mechanics and Physics of Solids",
volume = "39",
number = "1",
pages = "87 - 112",
year = "1991",
note = "",
issn = "0022-5096",
doi = "http://dx.doi.org/10.1016/0022-5096(91)90032-J",
url = "http://www.sciencedirect.com/science/article/pii/002250969190032J",
author = "Sanjay Govindjee and Juan Simo",
}

@article{gent92,
  title={Elasticity},
  author={Gent, AN},
  journal={Engineering With Rubber How to Design Rubber Components},
  pages={33--66},
  year={1992},
  publisher={Carl Hanser, Munich, Germany}
}
@article{ricard11,
  title={The collagen family},
  author={Ricard-Blum, Sylvie},
  journal={Cold Spring Harbor perspectives in biology},
  volume={3},
  number={1},
  pages={a004978},
  year={2011},
  publisher={Cold Spring Harbor Lab}
}

@article{Göktepe05,
title = "A micro–macro approach to rubber-like materials. Part III: The micro-sphere model of anisotropic Mullins-type damage ",
journal = "Journal of the Mechanics and Physics of Solids ",
volume = "53",
number = "10",
pages = "2259 - 2283",
year = "2005",
note = "",
issn = "0022-5096",
doi = "http://doi.org/10.1016/j.jmps.2005.04.010",
url = "http://www.sciencedirect.com/science/article/pii/S002250960500092X",
author = "Serdar Göktepe and Christian Miehe",
}

@article{Diani06,
title = "A damage directional constitutive model for Mullins effect with permanent set and induced anisotropy",
journal = "European Journal of Mechanics - A/Solids",
volume = "25",
number = "3",
pages = "483 - 496",
year = "2006",
note = "",
issn = "0997-7538",
doi = "http://dx.doi.org/10.1016/j.euromechsol.2005.09.011",
url = "http://www.sciencedirect.com/science/article/pii/S0997753805001397",
author = "J. Diani and M. Brieu and J.M. Vacherand",
}

@Article{Rajagopal16,
author="Rajagopal, K. R.
and Srinivasa, A. R.",
title="An implicit three-dimensional model for describing the inelastic response of solids undergoing finite deformation",
journal="Zeitschrift f{\"u}r angewandte Mathematik und Physik",
year="2016",
volume="67",
number="4",
pages="86",
issn="1420-9039",
doi="10.1007/s00033-016-0671-x",
url="http://dx.doi.org/10.1007/s00033-016-0671-x"
}

@article{merckel13,
  title={Constitutive modeling of the anisotropic behavior of Mullins softened filled rubbers},
  author={Merckel, Yannick and Diani, Julie and Brieu, Mathias and Caillard, Julien},
  journal={Mechanics of Materials},
  volume={57},
  pages={30--41},
  year={2013},
  publisher={Elsevier}
}
@Inbook{Cheng09,
author="Cheng, I-Chun
and Wagner, Sigurd",
editor="Wong, William S.
and Salleo, Alberto",
title="Overview of Flexible Electronics Technology",
bookTitle="Flexible Electronics: Materials and Applications",
year="2009",
publisher="Springer US",
address="Boston, MA",
pages="1--28",
isbn="978-0-387-74363-9",
doi="10.1007/978-0-387-74363-9_1",
url="http://dx.doi.org/10.1007/978-0-387-74363-9_1"
}

@article {Webbe15,
	author = {Webb, R. Chad and Ma, Yinji and Krishnan, Siddharth and Li, Yuhang and Yoon, Stephen and Guo, Xiaogang and Feng, Xue and Shi, Yan and Seidel, Miles and Cho, Nam Heon and Kurniawan, Jonas and Ahad, James and Sheth, Niral and Kim, Joseph and Taylor VI, James G. and Darlington, Tom and Chang, Ken and Huang, Weizhong and Ayers, Joshua and Gruebele, Alexander and Pielak, Rafal M. and Slepian, Marvin J. and Huang, Yonggang and Gorbach, Alexander M. and Rogers, John A.},
	title = {Epidermal devices for noninvasive, precise, and continuous mapping of macrovascular and microvascular blood flow},
	volume = {1},
	number = {9},
	year = {2015},
	doi = {10.1126/sciadv.1500701},
	publisher = {American Association for the Advancement of Science},
	URL = {http://advances.sciencemag.org/content/1/9/e1500701},
	eprint = {http://advances.sciencemag.org/content/1/9/e1500701.full.pdf},
	journal = {Science Advances}
}


@article {Rogers10,
	author = {Rogers, John A. and Someya, Takao and Huang, Yonggang},
	title = {Materials and Mechanics for Stretchable Electronics},
	volume = {327},
	number = {5973},
	pages = {1603--1607},
	year = {2010},
	doi = {10.1126/science.1182383},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/327/5973/1603},
	eprint = {http://science.sciencemag.org/content/327/5973/1603.full.pdf},
	journal = {Science}
}

@article{Zhao17,
  title={Mechanisms and Materials of Flexible and Stretchable Skin Sensors},
  author={Zhao, Yicong and Huang, Xian},
  journal={Micromachines},
  volume={8},
  number={3},
  pages={69},
  year={2017},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article {Xu14,
	author = {Xu, Sheng and Zhang, Yihui and Jia, Lin and Mathewson, Kyle E. and Jang, Kyung-In and Kim, Jeonghyun and Fu, Haoran and Huang, Xian and Chava, Pranav and Wang, Renhan and Bhole, Sanat and Wang, Lizhe and Na, Yoon Joo and Guan, Yue and Flavin, Matthew and Han, Zheshen and Huang, Yonggang and Rogers, John A.},
	title = {Soft Microfluidic Assemblies of Sensors, Circuits, and Radios for the Skin},
	volume = {344},
	number = {6179},
	pages = {70--74},
	year = {2014},
	doi = {10.1126/science.1250169},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/344/6179/70},
	eprint = {http://science.sciencemag.org/content/344/6179/70.full.pdf},
	journal = {Science}
}

@article{Shergold06,
title = "The uniaxial stress versus strain response of pig skin and silicone rubber at low and high strain rates ",
journal = "International Journal of Impact Engineering ",
volume = "32",
number = "9",
pages = "1384 - 1402",
year = "2006",
note = "",
issn = "0734-743X",
doi = "http://dx.doi.org/10.1016/j.ijimpeng.2004.11.010",
url = "http://www.sciencedirect.com/science/article/pii/S0734743X04002325",
author = "Oliver A. Shergold and Norman A. Fleck and Darren Radford",
}

@article{lim11,
  title={Mechanical response of pig skin under dynamic tensile loading},
  author={Lim, Jaeyoung and Hong, Jihye and Chen, Weinong W and Weerasooriya, Tusit},
  journal={International Journal of Impact Engineering},
  volume={38},
  number={2},
  pages={130--135},
  year={2011},
  publisher={Elsevier}
}

@book{fung13,
  title={Biomechanics: mechanical properties of living tissues},
  author={Fung, Yuan-cheng},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{Rey14,
title = "An original architectured NiTi silicone rubber structure for biomedical applications ",
journal = "Materials Science and Engineering: C ",
volume = "45",
number = "",
pages = "184 - 190",
year = "2014",
note = "",
issn = "0928-4931",
doi = "http://dx.doi.org/10.1016/j.msec.2014.08.062",
url = "http://www.sciencedirect.com/science/article/pii/S0928493114005578",
author = "T. Rey and J.-B. Le Cam and G. Chagnon and D. Favier and M. Rebouah and F. Razan and E. Robin and P. Didier and L. Heller and S. Faure and K. Janouchova",
}

@article {Amin10,
author = {Amin, A.F.M.S. and Lion, A. and Höfer, P.},
title = {Effect of temperature history on the mechanical behaviour of a filler-reinforced NR/BR blend: literature review and critical experiments},
journal = {ZAMM - Journal of Applied Mathematics and Mechanics / Zeitschrift für Angewandte Mathematik und Mechanik},
volume = {90},
number = {5},
publisher = {WILEY-VCH Verlag},
issn = {1521-4001},
url = {http://dx.doi.org/10.1002/zamm.200900365},
doi = {10.1002/zamm.200900365},
pages = {347--369},
keywords = {Mullins effect, healing, strain rate effect, crystallization, melting.},
year = {2010},
}

@article{Bouasse03,
author = {Bouasse, H., Carrière, Z.},
journal = {Annales de la Faculté des sciences de Toulouse : Mathématiques},
language = {fre},
number = {3},
pages = {257-283},
publisher = {GAUTHIER-VILLARS, IMPRIMEUR-EDITEUR ; ED. PRIVAT, IMPRIMEUR-LIBRAIRE},
title = {Sur les courbes de traction du caoutchouc vulcanisé},
url = {http://eudml.org/doc/72760},
volume = {5},
year = {1903},
}


@article{Holt32,
author = { W. L.   Holt },
title = {Behavior of Rubber under Repeated Stresses},
journal = {Rubber Chemistry and Technology},
volume = {5},
number = {1},
pages = {79-89},
year = {1932},
doi = {10.5254/1.3539319},
}

@article{Blanchard52,
author = {A. F. Blanchard and D. Parkinson},
title = {Breakage of Carbon-Rubber Networks by Applied Stress},
journal = {Industrial \& Engineering Chemistry},
volume = {44},
number = {4},
pages = {799-812},
year = {1952},
doi = {10.1021/ie50508a034},
}

@article{Mullins69,
author = { L.   Mullins },
title = {Softening of Rubber by Deformation},
journal = {Rubber Chemistry and Technology},
volume = {42},
number = {1},
pages = {339-362},
year = {1969},
}

@article {Harwood66,
author = {Harwood, J. A. C. and Payne, A. R.},
title = {Stress softening in natural rubber vulcanizates. Part IV. Unfilled vulcanizates},
journal = {Journal of Applied Polymer Science},
volume = {10},
number = {8},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
pages = {1203--1211},
year = {1966},
}


@article{Mullins49,
author = { L.   Mullins },
title = {Permanent Set in Vulcanized Rubber},
journal = {Rubber Chemistry and Technology},
volume = {22},
number = {4},
pages = {1036-1044},
year = {1949},
doi = {10.5254/1.3543010},
URL = { 
        http://dx.doi.org/10.5254/1.3543010  
},
}

@article{Blanchard52,
author = {Blanchard, A. F. and Parkinson, D.},
title = {Breakage of Carbon-Rubber Networks by Applied Stress},
journal = {Industrial \& Engineering Chemistry},
volume = {44},
number = {4},
pages = {799-812},
year = {1952},
doi = {10.1021/ie50508a034},

URL = { 
        http://dx.doi.org/10.1021/ie50508a034
},
}

@article{Houwink55,
author = { R.   Houwink },
title = {Slipping of Molecules during the Deformation of Reinforced Rubber},
journal = {Rubber Chemistry and Technology},
volume = {29},
number = {3},
pages = {888-893},
year = {1955},
doi = {10.5254/1.3542602},
}

@article {Kraus66,
author = {Kraus, G. and Childers, C. W. and Rollmann, K. W.},
title = {Stress softening in carbon black-reinforced vulcanizates. Strain rate and temperature effects},
journal = {Journal of Applied Polymer Science},
volume = {10},
number = {2},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
issn = {1097-4628},
url = {http://dx.doi.org/10.1002/app.1966.070100205},
doi = {10.1002/app.1966.070100205},
pages = {229--244},
year = {1966},
}

@article{Hanson05,
title = "Stress softening experiments in silica-filled polydimethylsiloxane provide insight into a mechanism for the Mullins effect ",
journal = "Polymer ",
volume = "46",
number = "24",
pages = "10989 - 10995",
year = "2005",
note = "",
issn = "0032-3861",
doi = "http://dx.doi.org/10.1016/j.polymer.2005.09.039",
author = "David E. Hanson and Marilyn Hawley and Robert Houlton and Kiran Chitanvis and Philip Rae and E. Bruce Orler and Debra A. Wrobleski",
}

@article {Fukahori05,
author = {Fukahori, Yoshihide},
title = {New progress in the theory and model of carbon black reinforcement of elastomers},
journal = {Journal of Applied Polymer Science},
volume = {95},
number = {1},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
issn = {1097-4628},
doi = {10.1002/app.20802},
pages = {60--67},
keywords = {carbon black, reinforcement, elastomers, interface model, crazing},
year = {2005},
}

@article{Haut89,
  title={The effects of orientation and location on the strength of dorsal rat skin in high and low speed tensile failure experiments},
  author={Haut, RC},
  journal={Journal of biomechanical engineering},
  volume={111},
  number={2},
  pages={136--140},
  year={1989},
  publisher={American Society of Mechanical Engineers}
}

@article{Dombi93,
title = "Correlation of High-Speed Tensile Strength with Collagen Content in Control and Lathyritic Rat Skin",
journal = "Journal of Surgical Research",
volume = "54",
number = "1",
pages = "21 - 28",
year = "1993",
note = "",
issn = "0022-4804",
doi = "http://dx.doi.org/10.1006/jsre.1993.1004",
url = "http://www.sciencedirect.com/science/article/pii/S0022480483710048",
author = "George W. Dombi and Roger C. Haut and Walter G. Sullivan",

}

@book{swaim90,
  title={Small animal wound management.},
  author={Swaim, Steven F and Henderson, Ralph A and Pidgeon, Rhoda S and others},
  year={1990},
  publisher={Lea \& Febiger}
}

@article{Annaidh12,
title = "Characterization of the anisotropic mechanical properties of excised human skin ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "5",
number = "1",
pages = "139 - 148",
year = "2012",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2011.08.016",
url = "http://www.sciencedirect.com/science/article/pii/S1751616111002219",
author = "Aisling Ní Annaidh and Karine Bruyère and Michel Destrade and Michael D. Gilchrist and Mélanie Otténio",
} 

@article{Munoz08,
title = "An experimental study of the mouse skin behaviour: Damage and inelastic aspects ",
journal = "Journal of Biomechanics ",
volume = "41",
number = "1",
pages = "93 - 99",
year = "2008",
note = "",
issn = "0021-9290",
doi = "http://doi.org/10.1016/j.jbiomech.2007.07.013",
url = "http://www.sciencedirect.com/science/article/pii/S002192900700320X",
author = "M.J. Muñoz and J.A. Bea and J.F. Rodríguez and I. Ochoa and J. Grasa and A. Pérez del Palomar and P. Zaragoza and R. Osta and M. Doblaré",
}

@article{Kang11,
title = "Ratchetting of porcine skin under uniaxial cyclic loading ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "4",
number = "3",
pages = "498 - 506",
year = "2011",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2010.12.015",
url = "http://www.sciencedirect.com/science/article/pii/S1751616110001906",
author = "Guozheng Kang and Xinfeng Wu",
}


@book{Berardesca95,
  title={Bioengineering of the skin: methods and instrumentation},
  author={Berardesca, Enzo and Elsner, Peter and Wilhelm, Klaus-Peter and Maibach, Howard I},
  volume={3},
  year={1995},
  publisher={CRC Press}
}

@article {Zhou10,
	author = {Zhou, B. and Xu, F. and Chen, C. Q. and Lu, T. J.},
	title = {Strain rate sensitivity of skin tissue under thermomechanical loading},
	volume = {368},
	number = {1912},
	pages = {679--690},
	year = {2010},
	doi = {10.1098/rsta.2009.0238},
	publisher = {The Royal Society},
	issn = {1364-503X},
	URL = {http://rsta.royalsocietypublishing.org/content/368/1912/679},
	eprint = {http://rsta.royalsocietypublishing.org/content/368/1912/679.full.pdf},
	journal = {Philosophical Transactions of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

@article{lanir79,
  title={The rheological behavior of the skin: experimental results and a structural model.},
  author={Lanir, Y},
  journal={Biorheology},
  volume={16},
  number={3},
  pages={191},
  year={1979}
}

@article{Ottenio15,
title = "Strain rate and anisotropy effects on the tensile failure characteristics of human skin ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "41",
number = "",
pages = "241 - 250",
year = "2015",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2014.10.006",
url = "http://www.sciencedirect.com/science/article/pii/S1751616114003282",
author = "Mélanie Ottenio and Doris Tran and Aisling Ní Annaidh and Michael D. Gilchrist and Karine Bruyère",
}

@article{Tong76,
title = "The stress-strain relationship for the skin",
journal = "Journal of Biomechanics",
volume = "9",
number = "10",
pages = "649 - 657",
year = "1976",
note = "",
issn = "0021-9290",
doi = "http://dx.doi.org/10.1016/0021-9290(76)90107-X",
url = "http://www.sciencedirect.com/science/article/pii/002192907690107X",
author = "Pin Tong and Yuang-Cheng Fung",
}

@article{Danielson73,
  title={Human skin as an elastic membrane},
  author={Danielson, DA},
  journal={Journal of Biomechanics},
  volume={6},
  number={5},
  pages={539--546},
  year={1973},
  publisher={Elsevier}
}

@article{North78,
  title={Volume compressibility of human abdominal skin},
  author={North, James F and Gibson, Francis},
  journal={Journal of biomechanics},
  volume={11},
  number={4},
  pages={203207--205},
  year={1978},
  publisher={Elsevier}
}

@ARTICLE{Pena11,
author={Pena, E.},
title={Prediction of the softening and damage effects with permanent set in fibrous biological materials},
journal={Journal of the Mechanics and Physics of Solids},
year={2011},
volume={59},
number={9},
pages={1808-1822},
doi={10.1016/j.jmps.2011.05.013},
note={cited By 26},
document_type={Article},
source={Scopus},
}

@Article{Peña10,
author="Pe{\~{n}}a, Estefania
and Calvo, B.
and Mart{\'i}nez, M. A.
and Martins, P.
and Mascarenhas, T.
and Jorge, R. M. N.
and Ferreira, A.
and Doblar{\'e}, M.",
title="Experimental study and constitutive modeling of the viscoelastic mechanical properties of the human prolapsed vaginal tissue",
journal="Biomechanics and Modeling in Mechanobiology",
year="2010",
volume="9",
number="1",
pages="35--44",
issn="1617-7940",
doi="10.1007/s10237-009-0157-2",
url="http://dx.doi.org/10.1007/s10237-009-0157-2"
}

@Article{Ehret07,
author="Ehret, Alexander E.
and Itskov, Mikhail",
title="A polyconvex hyperelastic model for fiber-reinforced materials in application to soft tissues",
journal="Journal of Materials Science",
year="2007",
volume="42",
number="21",
pages="8853--8863",
issn="1573-4803",
doi="10.1007/s10853-007-1812-6",
url="http://dx.doi.org/10.1007/s10853-007-1812-6"
}

@article{Zhu16,
title = "Logarithmic rate based elasto-viscoplastic cyclic constitutive model for soft biological tissues ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "61",
number = "",
pages = "397 - 409",
year = "2016",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2016.03.014",
url = "http://www.sciencedirect.com/science/article/pii/S1751616116300340",
author = "Yilin Zhu and Guozheng Kang and Chao Yu and Leong Hien Poh",
}

@ARTICLE{Humphrey87,
author={Humphrey, J.D. and Yin, F.C.},
title={A new constitutive formulation for characterizing the mechanical behavior of soft tissues.},
journal={Biophysical Journal},
year={1987},
volume={52},
number={4},
pages={563-570},
note={cited By 66},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0023428314&partnerID=40&md5=87b13645541151e194b58a3a56fef4ea},
document_type={Article},
source={Scopus},
}

@Article{,
author="Rajagopal, K. R.
and Srinivasa, A. R.",
title="An implicit three-dimensional model for describing the inelastic response of solids undergoing finite deformation",
journal="Zeitschrift f{\"u}r angewandte Mathematik und Physik",
year="2016",
volume="67",
number="4",
pages="86",
doi="10.1007/s00033-016-0671-x",
url="http://dx.doi.org/10.1007/s00033-016-0671-x"
}


@article{Tonge13,
title = "Full-field bulge test for planar anisotropic tissues: Part \{II\} – A thin shell method for determining material parameters and comparison of two distributed fiber modeling approaches ",
journal = "Acta Biomaterialia ",
volume = "9",
number = "4",
pages = "5926 - 5942",
year = "2013",
note = "",
issn = "1742-7061",
doi = "http://doi.org/10.1016/j.actbio.2012.11.034",
url = "http://www.sciencedirect.com/science/article/pii/S1742706112005843",
author = "Theresa K. Tonge and Liming M. Voo and Thao D. Nguyen",
}


@Article{Carew00,
author="Carew, E. O.
and Barber, J. E.
and Vesely, I.",
title="Role of Preconditioning and Recovery Time in Repeated Testing of Aortic Valve Tissues: Validation Through Quasilinear Viscoelastic Theory",
journal="Annals of Biomedical Engineering",
year="2000",
volume="28",
number="9",
pages="1093--1100",
issn="1573-9686",
doi="10.1114/1.1310221",
url="http://dx.doi.org/10.1114/1.1310221"
}

@ARTICLE{Giles07,
author={Giles, J.M. and Black, A.E. and Bischoff, J.E.},
title={Anomalous rate dependence of the preconditioned response of soft tissue during load controlled deformation},
journal={Journal of Biomechanics},
year={2007},
volume={40},
number={4},
pages={777-785},
doi={10.1016/j.jbiomech.2006.03.017},
note={cited By 26},
document_type={Article},
source={Scopus},
}

@article{Schriefl15,
title = "Selective enzymatic removal of elastin and collagen from human abdominal aortas: Uniaxial mechanical response and constitutive modeling ",
journal = "Acta Biomaterialia ",
volume = "17",
number = "",
pages = "125 - 136",
year = "2015",
note = "",
issn = "1742-7061",
doi = "http://doi.org/10.1016/j.actbio.2015.01.003",
url = "http://www.sciencedirect.com/science/article/pii/S1742706115000045",
author = "Andreas J. Schriefl and Thomas Schmidt and Daniel Balzani and Gerhard Sommer and Gerhard A. Holzapfel",
}

@article{Peña09,
title = "On the Mullins effect and hysteresis of fibered biological materials: A comparison between continuous and discontinuous damage models ",
journal = "International Journal of Solids and Structures ",
volume = "46",
number = "7–8",
pages = "1727 - 1735",
year = "2009",
note = "",
issn = "0020-7683",
doi = "http://doi.org/10.1016/j.ijsolstr.2008.12.015",
url = "http://www.sciencedirect.com/science/article/pii/S0020768308005179",
author = "Estefanía Peña and Juan A. Peña and Manuel Doblaré",
}


@article{MEIJER99,
author = { R.   MEIJER  and  L. F. A.   DOUVEN  and  C. W. J.   OOMENS },
title = {Characterisation of Anisotropic and Non-linear Behaviour of Human Skin In Vivo},
journal = {Computer Methods in Biomechanics and Biomedical Engineering},
volume = {2},
number = {1},
pages = {13-27},
year = {1999},
doi = {10.1080/10255849908907975},
    note ={PMID: 11264815},
}

@article{Sasso08,
title = "Characterization of hyperelastic rubber-like materials by biaxial and uniaxial stretching tests based on optical methods ",
journal = "Polymer Testing ",
volume = "27",
number = "8",
pages = "995 - 1004",
year = "2008",
note = "",
issn = "0142-9418",
doi = "https://doi.org/10.1016/j.polymertesting.2008.09.001",
url = "http://www.sciencedirect.com/science/article/pii/S0142941808001529",
author = "M. Sasso and G. Palmieri and G. Chiappini and D. Amodio",
}

@article{lanir74,
  title={Two-dimensional mechanical properties of rabbit skin—II. Experimental results},
  author={Lanir, Y and Fung, YC},
  journal={Journal of biomechanics},
  volume={7},
  number={2},
  pages={171IN9175--174182},
  year={1974},
  publisher={Elsevier}
}

@Article{Sacks00,
author="Sacks, Michael S.",
title="Biaxial Mechanical Evaluation of Planar Biological Materials",
journal="Journal of elasticity and the physical science of solids",
year="2000",
volume="61",
number="1",
pages="199",
issn="1573-2681",
doi="10.1023/A:1010917028671",
url="http://dx.doi.org/10.1023/A:1010917028671"
}

@article{lokshin09,
  title={Viscoelasticity and preconditioning of rat skin under uniaxial stretch: microstructural constitutive characterization},
  author={Lokshin, Olga and Lanir, Yoram},
  journal={Journal of biomechanical engineering},
  volume={131},
  number={3},
  pages={031009},
  year={2009},
  publisher={American Society of Mechanical Engineers}
}

@article {Rivlin51,
	author = {Rivlin, R. S. and Saunders, D. W.},
	title = {Large Elastic Deformations of Isotropic Materials. VII. Experiments on the Deformation of Rubber},
	volume = {243},
	number = {865},
	pages = {251--288},
	year = {1951},
	doi = {10.1098/rsta.1951.0004},
	publisher = {The Royal Society},
	issn = {0080-4614},
	URL = {http://rsta.royalsocietypublishing.org/content/243/865/251},
	eprint = {http://rsta.royalsocietypublishing.org/content/243/865/251.full.pdf},
	journal = {Philosophical Transactions of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

@article{obata70,
  title={Mechanical properties of natural rubber vulcanizates in finite deformation},
  author={Obata, Yutaka and Kawabata, Sueo and Kawai, Hiromichi},
  journal={Journal of Polymer Science Part A-2: Polymer Physics},
  volume={8},
  number={6},
  pages={903--919},
  year={1970},
  publisher={Wiley Online Library}
}

@inproceedings{korochkina05,
  title={Choosing constitutive models for elastomers used in printing processes},
  author={Korochkina, TV and Claypole, TC and Gethin, DT},
  booktitle={CONSTITUTIVE MODELS FOR RUBBER-PROCEEDINGS-},
  volume={4},
  pages={431},
  year={2005},
  organization={Balkema}
}

@Article{Wineman15,
author="Wineman, Alan
and Rajagopal, K. R.",
title="A constitutive theory for multi-functional fiber reinforced composites",
journal="Acta Mechanica",
year="2015",
volume="226",
number="8",
pages="2671--2679",
issn="1619-6937",
doi="10.1007/s00707-015-1345-z",
url="http://dx.doi.org/10.1007/s00707-015-1345-z"
}

@article{ayoub16,
  title={Heart valve biomechanics and underlying mechanobiology},
  author={Ayoub, Salma and Ferrari, Giovanni and Gorman, Robert C and Gorman, Joseph H and Schoen, Frederick J and Sacks, Michael S},
  journal={Comprehensive Physiology},
  year={2016},
  publisher={Wiley Online Library}
}

@article{frisen69,
  title={Rheological analysis of soft collagenous tissue: Part I: Theoretical considerations},
  author={Frisen, M and M{\"a}gi, M and Sonnerup, L and Viidik, A},
  journal={Journal of Biomechanics},
  volume={2},
  number={1},
  pages={13--20},
  year={1969},
  publisher={Elsevier}
}

@article{frisen1969b,
  title={Rheological analysis of soft collagenous tissue: Part II: Experimental evaluations and verifications},
  author={Frisen, M and M{\"a}gi, M and Sonnerup, L and Viidik, A},
  journal={Journal of biomechanics},
  volume={2},
  number={1},
  pages={21--28},
  year={1969},
  publisher={Elsevier}
}

@article{sacks03,
  title={Incorporation of experimentally-derived fiber orientation into a structural constitutive model for planar collagenous tissues},
  author={Sacks, Michael S and others},
  journal={TRANSACTIONS-AMERICAN SOCIETY OF MECHANICAL ENGINEERS JOURNAL OF BIOMECHANICAL ENGINEERING},
  volume={125},
  number={2},
  pages={280--287},
  year={2003},
  publisher={AMERICAN SOCIETY MECHANICAL ENGINEERS}
}

@article{sellaro07,
  title={Effects of collagen fiber orientation on the response of biologically derived soft tissue biomaterials to cyclic loading},
  author={Sellaro, Tiffany L and Hildebrand, Daniel and Lu, Qijin and Vyavahare, Naren and Scott, Michael and Sacks, Michael S},
  journal={Journal of Biomedical Materials Research Part A},
  volume={80},
  number={1},
  pages={194--205},
  year={2007},
  publisher={Wiley Online Library}
}

@Article{Freed16,
author="Freed, Alan D.
and Rajagopal, K. R.",
title="A promising approach for modeling biological fibers",
journal="Acta Mechanica",
year="2016",
month="Jun",
day="01",
volume="227",
number="6",
pages="1609--1619",
}


@article{Zhang16,
title = "A meso-scale layer-specific structural constitutive model of the mitral heart valve leaflets",
journal = "Acta Biomaterialia",
volume = "32",
number = "Supplement C",
pages = "238 - 255",
year = "2016",
issn = "1742-7061",
doi = "https://doi.org/10.1016/j.actbio.2015.12.001",
url = "http://www.sciencedirect.com/science/article/pii/S1742706115302397",
author = "Will Zhang and Salma Ayoub and Jun Liao and Michael S. Sacks",
}

@ARTICLE{Pena11,
author={Pena, E.},
title={Prediction of the softening and damage effects with permanent set in fibrous biological materials},
journal={Journal of the Mechanics and Physics of Solids},
year={2011},
volume={59},
number={9},
pages={1808-1822},
doi={10.1016/j.jmps.2011.05.013},
note={cited By 26},
document_type={Article},
source={Scopus},
}

@Article{Pena10,
author="Pe{\~{n}}a, Estefania
and Calvo, B.
and Mart{\'i}nez, M. A.
and Martins, P.
and Mascarenhas, T.
and Jorge, R. M. N.
and Ferreira, A.
and Doblar{\'e}, M.",
title="Experimental study and constitutive modeling of the viscoelastic mechanical properties of the human prolapsed vaginal tissue",
journal="Biomechanics and Modeling in Mechanobiology",
year="2010",
volume="9",
number="1",
pages="35--44",
issn="1617-7940",
doi="10.1007/s10237-009-0157-2",
url="http://dx.doi.org/10.1007/s10237-009-0157-2"
}


@article{Pena09,
title = "On the Mullins effect and hysteresis of fibered biological materials: A comparison between continuous and discontinuous damage models ",
journal = "International Journal of Solids and Structures ",
volume = "46",
number = "7–8",
pages = "1727 - 1735",
year = "2009",
note = "",
issn = "0020-7683",
doi = "http://doi.org/10.1016/j.ijsolstr.2008.12.015",
url = "http://www.sciencedirect.com/science/article/pii/S0020768308005179",
author = "Estefanía Peña and Juan A. Peña and Manuel Doblaré",
}


@article{LIAO99,
title = "A failure model for ligaments",
journal = "Journal of Biomechanics",
volume = "32",
number = "2",
pages = "183 - 188",
year = "1999",
issn = "0021-9290",
doi = "https://doi.org/10.1016/S0021-9290(98)00169-9",
url = "http://www.sciencedirect.com/science/article/pii/S0021929098001699",
author = "Hongyan Liao and Stephen M. Belkoff",
keywords = "Failure, Structural model, Collagen, Ligament"
}

@article{HILL12,
title = "A theoretical and non-destructive experimental approach for direct inclusion of measured collagen orientation and recruitment into mechanical models of the artery wall",
journal = "Journal of Biomechanics",
volume = "45",
number = "5",
pages = "762 - 771",
year = "2012",
note = "Special Issue on Cardiovascular Solid Mechanics",
issn = "0021-9290",
doi = "https://doi.org/10.1016/j.jbiomech.2011.11.016",
url = "http://www.sciencedirect.com/science/article/pii/S0021929011006981",
author = "Michael R. Hill and Xinjie Duan and Gregory A. Gibson and Simon Watkins and Anne M. Robertson",
keywords = "Collagen fiber, Collagen recruitment, Orientation distribution function, Uniaxial testing, Multi-photon microscopy"
}

@article{Benias18,
  title={Structure and Distribution of an Unrecognized Interstitium in Human Tissues},
  author={Benias, Petros C and Wells, Rebecca G and Sackey-Aboagye, Bridget and Klavan, Heather and Reidy, Jason and Buonocore, Darren and Miranda, Markus and Kornacki, Susan and Wayne, Michael and Carr-Locke, David L and others},
  journal={Scientific reports},
  volume={8},
  number={1},
  pages={4947},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{Mullin48,
author = { L.   Mullins },
title = {Effect of Stretching on the Properties of Rubber},
journal = {Rubber Chemistry and Technology},
volume = {21},
number = {2},
pages = {281-300},
year = {1948},
doi = {10.5254/1.3546914},
URL = { https://doi.org/10.5254/1.3546914},
eprint = { https://doi.org/10.5254/1.3546914}
}


@article{XU08,
title = "Biothermomechanics of skin tissues",
journal = "Journal of the Mechanics and Physics of Solids",
volume = "56",
number = "5",
pages = "1852 - 1884",
year = "2008",
issn = "0022-5096",
doi = "https://doi.org/10.1016/j.jmps.2007.11.011",
url = "http://www.sciencedirect.com/science/article/pii/S002250960700227X",
author = "F. Xu and T.J. Lu and K.A. Seffen",
keywords = "Skin tissue, Biothermomechanics, Analytical model, Numerical method, Thermal"
}

@article{Afsar18,
title = "Inelastic Response of Skin under Uniaxial Cyclic Mechanical Loading-Multinetwork Model Comparison with Experiments ",
journal = "International Journal of Engineering Science",
volume = "",
number = "",
pages = "",
year = "Under Review",
note = "",
issn = "",
doi = "",
url = "",
author = "N. Afsar Kazerooni and A.R. Srinivasa and J.C. Criscione"
}

@article{Zhu14,
title = "A finite viscoelastic–plastic model for describing the uniaxial ratchetting of soft biological tissues",
journal = "Journal of Biomechanics",
volume = "47",
number = "5",
pages = "996 - 1003",
year = "2014",
issn = "0021-9290",
doi = "https://doi.org/10.1016/j.jbiomech.2014.01.004",
url = "http://www.sciencedirect.com/science/article/pii/S0021929014000177",
author = "Yilin Zhu and Guozheng Kang and Qianhua Kan and Chao Yu",
keywords = "Soft biological tissues, Constitutive model, Anisotropy, Ratchetting, Time-dependence"
}

@article{LOKSHIN091,
title = "Micro and macro rheology of planar tissues",
journal = "Biomaterials",
volume = "30",
number = "17",
pages = "3118 - 3127",
year = "2009",
issn = "0142-9612",
doi = "https://doi.org/10.1016/j.biomaterials.2009.02.039",
url = "http://www.sciencedirect.com/science/article/pii/S0142961209002312",
author = "Olga Lokshin and Yoram Lanir",
}

@InProceedings{Nava04,
author="Nava, Alessandro
and Mazza, Edoardo
and Haefner, Oliver
and Bajka, Michael",
editor="Cotin, St{\'e}phane
and Metaxas, Dimitris",
title="Experimental Observation and Modelling of Preconditioning in Soft Biological Tissues",
booktitle="Medical Simulation",
year="2004",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="1--8",
isbn="978-3-540-25968-8"
}

@article{Avis00,
author = {N. J. Avis},
title = {Virtual environment technologies},
journal = {Minimally Invasive Therapy \& Allied Technologies},
volume = {9},
number = {5},
pages = {333-339},
year  = {2000},
publisher = {Taylor & Francis},
doi = {10.3109/13645700009061455},
}

@article{Satava99,
  title={Virtual reality in medicine},
  author={Satava, Richard M and others},
  journal={Bmj},
  volume={319},
  number={7220},
  pages={1305},
  year={1999},
  publisher={British Medical Journal Publishing Group}
}


@Article{Eshel01,
author="Eshel, H.
and Lanir, Y.",
title="Effects of Strain Level and Proteoglycan Depletion on Preconditioning and Viscoelastic Responses of Rat Dorsal Skin",
journal="Annals of Biomedical Engineering",
year="2001",
month="Feb",
day="01",
volume="29",
number="2",
pages="164--172",
issn="1573-9686",
}

@book{srinivasa09,
  title={Inelasticity of materials: an engineering approach and a practical guide},
  author={Srinivasa, Arun R and Srinivasan, Sivakumar M},
  volume={80},
  year={2009},
  publisher={World Scientific Publishing Company}
}





==> reference.tex <==

@article{Mullins48,
title = {Effect of Stretching on the Properties of Rubber},
journal = {Rubber Chemistry and Technology},
volume = {21},
number = {2},
pages = {281-300},
year = {1948},
doi = {10.5254/1.3546914},
URL = {http://dx.doi.org/10.5254/1.3546914   },
eprint = { http://dx.doi.org/10.5254/1.3546914  }
}

@inbook{McGrath10,
author = {J. A. McGrath and J. Uitto},
publisher = {Wiley-Blackwell},
isbn = {9781444317633},
title = {Anatomy and Organization of Human Skin},
booktitle = {Rook's Textbook of Dermatology},
chapter = {3},
pages = {1-53},
doi = {10.1002/9781444317633.ch3},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/9781444317633.ch3},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/9781444317633.ch3},
year = {2010},
}


@article{Naylor11,
title = "Molecular aspects of skin ageing ",
journal = "Maturitas ",
volume = "69",
number = "3",
pages = "249 - 256",
year = "2011",
note = "",
issn = "0378-5122",
doi = "http://dx.doi.org/10.1016/j.maturitas.2011.04.011",
url = "http://www.sciencedirect.com/science/article/pii/S0378512211001496",
author = "Elizabeth C. Naylor and Rachel E.B. Watson and Michael J. Sherratt",
}

@article{Minns73,
title = "The role of the fibrous components and ground substance in the mechanical properties of biological tissues: A preliminary investigation ",
journal = "Journal of Biomechanics ",
volume = "6",
number = "2",
pages = "153 - 165",
year = "1973",
note = "",
issn = "0021-9290",
doi = "http://dx.doi.org/10.1016/0021-9290(73)90084-5",
url = "http://www.sciencedirect.com/science/article/pii/0021929073900845",
author = "R.J. Minns and P.D. Soden and D.S. Jackson"
}

@article{Brown73,
title={A scanning electron microscope study of the effects of uniaxial tension on human skin},
author={Brown, Ian A},
journal={British Journal of Dermatology},
volume={89},
number={4},
pages={383--393},
year={1973},
publisher={Wiley Online Library}
}

@Inbook{Xu11,
author="Xu, Feng
and Lu, Tianjian",
title="Skin Mechanical Behaviour",
bookTitle="Introduction to Skin Biothermomechanics and Thermal Pain",
year="2011",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
chapter="5",
pages="87-104",
isbn="978-3-642-13202-5",
doi="10.1007/978-3-642-13202-5_5",
url="https://doi.org/10.1007/978-3-642-13202-5_5"
}


@article{OXLUND88,
title = "The role of elastin in the mechanical properties of skin",
journal = "Journal of Biomechanics",
volume = "21",
number = "3",
pages = "213 - 218",
year = "1988",
note = "",
issn = "0021-9290",
doi = "http://dx.doi.org/10.1016/0021-9290(88)90172-8",
url = "http://www.sciencedirect.com/science/article/pii/0021929088901728",
author = "Hans Oxlund and Jan Manschot and A. Viidik",
}


@article{Diani09,
  title={A review on the Mullins effect},
  author={Diani, Julie and Fayolle, Bruno and Gilormini, Pierre},
  journal={European Polymer Journal},
  volume={45},
  number={3},
  pages={601--612},
  year={2009},
  publisher={Elsevier}
}

@article{lion96,
  title={A constitutive model for carbon black filled rubber: experimental investigations and mathematical representation},
  author={Lion, Alexander},
  journal={Continuum Mechanics and Thermodynamics},
  volume={8},
  number={3},
  pages={153--169},
  year={1996},
  publisher={Springer}
}


@article{Treloar44,
author = { L. R. G.   Treloar },
title = {The Elasticity of a Network of Long-Chain Molecules. II},
journal = {Rubber Chemistry and Technology},
volume = {17},
number = {2},
pages = {296-302},
year = {1944},
doi = {10.5254/1.3546653},
URL = {http://dx.doi.org/10.5254/1.3546653},
eprint = { http://dx.doi.org/10.5254/1.3546653}
}


@article{Simo87,
title = "On a fully three-dimensional finite-strain viscoelastic damage model: Formulation and computational aspects",
journal = "Computer Methods in Applied Mechanics and Engineering",
volume = "60",
number = "2",
pages = "153 - 173",
year = "1987",
note = "",
issn = "0045-7825",
doi = "http://dx.doi.org/10.1016/0045-7825(87)90107-1",
url = "http://www.sciencedirect.com/science/article/pii/0045782587901071",
author = "J.C. Simo",
}

@article{miehe95,
  title={Discontinuous and continuous damage evolution in Ogden-type large-strain elastic materials},
  author={Miehe, Ch},
  journal={European journal of mechanics. A. Solids},
  volume={14},
  number={5},
  pages={697--720},
  year={1995},
  publisher={Elsevier}
}
@article{Guth43,
author = {Hubert M. James and Eugene Guth},
title = {Theory of the Elastic Properties of Rubber},
journal = {The Journal of Chemical Physics},
volume = {11},
number = {10},
pages = {455-481},
year = {1943},
doi = {10.1063/1.1723785},
}

@article{Arruda93,
title = "A three-dimensional constitutive model for the large stretch behavior of rubber elastic materials",
journal = "Journal of the Mechanics and Physics of Solids",
volume = "41",
number = "2",
pages = "389 - 412",
year = "1993",
note = "",
issn = "0022-5096",
doi = "http://dx.doi.org/10.1016/0022-5096(93)90013-6",
url = "http://www.sciencedirect.com/science/article/pii/0022509693900136",
author = "Ellen M. Arruda and Mary C. Boyce",
}

@article{Govindjee91,
title = "A micro-mechanically based continuum damage model for carbon black-filled rubbers incorporating Mullins' effect",
journal = "Journal of the Mechanics and Physics of Solids",
volume = "39",
number = "1",
pages = "87 - 112",
year = "1991",
note = "",
issn = "0022-5096",
doi = "http://dx.doi.org/10.1016/0022-5096(91)90032-J",
url = "http://www.sciencedirect.com/science/article/pii/002250969190032J",
author = "Sanjay Govindjee and Juan Simo",
}

@article{gent92,
  title={Elasticity},
  author={Gent, AN},
  journal={Engineering With Rubber How to Design Rubber Components},
  pages={33--66},
  year={1992},
  publisher={Carl Hanser, Munich, Germany}
}
@article{ricard11,
  title={The collagen family},
  author={Ricard-Blum, Sylvie},
  journal={Cold Spring Harbor perspectives in biology},
  volume={3},
  number={1},
  pages={a004978},
  year={2011},
  publisher={Cold Spring Harbor Lab}
}

@article{Göktepe05,
title = "A micro–macro approach to rubber-like materials. Part III: The micro-sphere model of anisotropic Mullins-type damage ",
journal = "Journal of the Mechanics and Physics of Solids ",
volume = "53",
number = "10",
pages = "2259 - 2283",
year = "2005",
note = "",
issn = "0022-5096",
doi = "http://doi.org/10.1016/j.jmps.2005.04.010",
url = "http://www.sciencedirect.com/science/article/pii/S002250960500092X",
author = "Serdar Göktepe and Christian Miehe",
}

@article{Diani06,
title = "A damage directional constitutive model for Mullins effect with permanent set and induced anisotropy",
journal = "European Journal of Mechanics - A/Solids",
volume = "25",
number = "3",
pages = "483 - 496",
year = "2006",
note = "",
issn = "0997-7538",
doi = "http://dx.doi.org/10.1016/j.euromechsol.2005.09.011",
url = "http://www.sciencedirect.com/science/article/pii/S0997753805001397",
author = "J. Diani and M. Brieu and J.M. Vacherand",
}

@Article{Rajagopal16,
author="Rajagopal, K. R.
and Srinivasa, A. R.",
title="An implicit three-dimensional model for describing the inelastic response of solids undergoing finite deformation",
journal="Zeitschrift f{\"u}r angewandte Mathematik und Physik",
year="2016",
volume="67",
number="4",
pages="86",
issn="1420-9039",
doi="10.1007/s00033-016-0671-x",
url="http://dx.doi.org/10.1007/s00033-016-0671-x"
}

@article{merckel13,
  title={Constitutive modeling of the anisotropic behavior of Mullins softened filled rubbers},
  author={Merckel, Yannick and Diani, Julie and Brieu, Mathias and Caillard, Julien},
  journal={Mechanics of Materials},
  volume={57},
  pages={30--41},
  year={2013},
  publisher={Elsevier}
}
@Inbook{Cheng09,
author="Cheng, I-Chun
and Wagner, Sigurd",
editor="Wong, William S.
and Salleo, Alberto",
title="Overview of Flexible Electronics Technology",
bookTitle="Flexible Electronics: Materials and Applications",
year="2009",
publisher="Springer US",
address="Boston, MA",
pages="1--28",
isbn="978-0-387-74363-9",
doi="10.1007/978-0-387-74363-9_1",
url="http://dx.doi.org/10.1007/978-0-387-74363-9_1"
}

@article {Webbe15,
	author = {Webb, R. Chad and Ma, Yinji and Krishnan, Siddharth and Li, Yuhang and Yoon, Stephen and Guo, Xiaogang and Feng, Xue and Shi, Yan and Seidel, Miles and Cho, Nam Heon and Kurniawan, Jonas and Ahad, James and Sheth, Niral and Kim, Joseph and Taylor VI, James G. and Darlington, Tom and Chang, Ken and Huang, Weizhong and Ayers, Joshua and Gruebele, Alexander and Pielak, Rafal M. and Slepian, Marvin J. and Huang, Yonggang and Gorbach, Alexander M. and Rogers, John A.},
	title = {Epidermal devices for noninvasive, precise, and continuous mapping of macrovascular and microvascular blood flow},
	volume = {1},
	number = {9},
	year = {2015},
	doi = {10.1126/sciadv.1500701},
	publisher = {American Association for the Advancement of Science},
	URL = {http://advances.sciencemag.org/content/1/9/e1500701},
	eprint = {http://advances.sciencemag.org/content/1/9/e1500701.full.pdf},
	journal = {Science Advances}
}


@article {Rogers10,
	author = {Rogers, John A. and Someya, Takao and Huang, Yonggang},
	title = {Materials and Mechanics for Stretchable Electronics},
	volume = {327},
	number = {5973},
	pages = {1603--1607},
	year = {2010},
	doi = {10.1126/science.1182383},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/327/5973/1603},
	eprint = {http://science.sciencemag.org/content/327/5973/1603.full.pdf},
	journal = {Science}
}

@article{Zhao17,
  title={Mechanisms and Materials of Flexible and Stretchable Skin Sensors},
  author={Zhao, Yicong and Huang, Xian},
  journal={Micromachines},
  volume={8},
  number={3},
  pages={69},
  year={2017},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article {Xu14,
	author = {Xu, Sheng and Zhang, Yihui and Jia, Lin and Mathewson, Kyle E. and Jang, Kyung-In and Kim, Jeonghyun and Fu, Haoran and Huang, Xian and Chava, Pranav and Wang, Renhan and Bhole, Sanat and Wang, Lizhe and Na, Yoon Joo and Guan, Yue and Flavin, Matthew and Han, Zheshen and Huang, Yonggang and Rogers, John A.},
	title = {Soft Microfluidic Assemblies of Sensors, Circuits, and Radios for the Skin},
	volume = {344},
	number = {6179},
	pages = {70--74},
	year = {2014},
	doi = {10.1126/science.1250169},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/344/6179/70},
	eprint = {http://science.sciencemag.org/content/344/6179/70.full.pdf},
	journal = {Science}
}

@article{Shergold06,
title = "The uniaxial stress versus strain response of pig skin and silicone rubber at low and high strain rates ",
journal = "International Journal of Impact Engineering ",
volume = "32",
number = "9",
pages = "1384 - 1402",
year = "2006",
note = "",
issn = "0734-743X",
doi = "http://dx.doi.org/10.1016/j.ijimpeng.2004.11.010",
url = "http://www.sciencedirect.com/science/article/pii/S0734743X04002325",
author = "Oliver A. Shergold and Norman A. Fleck and Darren Radford",
}

@article{lim11,
  title={Mechanical response of pig skin under dynamic tensile loading},
  author={Lim, Jaeyoung and Hong, Jihye and Chen, Weinong W and Weerasooriya, Tusit},
  journal={International Journal of Impact Engineering},
  volume={38},
  number={2},
  pages={130--135},
  year={2011},
  publisher={Elsevier}
}

@book{fung13,
  title={Biomechanics: mechanical properties of living tissues},
  author={Fung, Yuan-cheng},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{Rey14,
title = "An original architectured NiTi silicone rubber structure for biomedical applications ",
journal = "Materials Science and Engineering: C ",
volume = "45",
number = "",
pages = "184 - 190",
year = "2014",
note = "",
issn = "0928-4931",
doi = "http://dx.doi.org/10.1016/j.msec.2014.08.062",
url = "http://www.sciencedirect.com/science/article/pii/S0928493114005578",
author = "T. Rey and J.-B. Le Cam and G. Chagnon and D. Favier and M. Rebouah and F. Razan and E. Robin and P. Didier and L. Heller and S. Faure and K. Janouchova",
}

@article {Amin10,
author = {Amin, A.F.M.S. and Lion, A. and Höfer, P.},
title = {Effect of temperature history on the mechanical behaviour of a filler-reinforced NR/BR blend: literature review and critical experiments},
journal = {ZAMM - Journal of Applied Mathematics and Mechanics / Zeitschrift für Angewandte Mathematik und Mechanik},
volume = {90},
number = {5},
publisher = {WILEY-VCH Verlag},
issn = {1521-4001},
url = {http://dx.doi.org/10.1002/zamm.200900365},
doi = {10.1002/zamm.200900365},
pages = {347--369},
keywords = {Mullins effect, healing, strain rate effect, crystallization, melting.},
year = {2010},
}

@article{Bouasse03,
author = {Bouasse, H., Carrière, Z.},
journal = {Annales de la Faculté des sciences de Toulouse : Mathématiques},
language = {fre},
number = {3},
pages = {257-283},
publisher = {GAUTHIER-VILLARS, IMPRIMEUR-EDITEUR ; ED. PRIVAT, IMPRIMEUR-LIBRAIRE},
title = {Sur les courbes de traction du caoutchouc vulcanisé},
url = {http://eudml.org/doc/72760},
volume = {5},
year = {1903},
}


@article{Holt32,
author = { W. L.   Holt },
title = {Behavior of Rubber under Repeated Stresses},
journal = {Rubber Chemistry and Technology},
volume = {5},
number = {1},
pages = {79-89},
year = {1932},
doi = {10.5254/1.3539319},
}

@article{Blanchard52,
author = {A. F. Blanchard and D. Parkinson},
title = {Breakage of Carbon-Rubber Networks by Applied Stress},
journal = {Industrial \& Engineering Chemistry},
volume = {44},
number = {4},
pages = {799-812},
year = {1952},
doi = {10.1021/ie50508a034},
}

@article{Mullins69,
author = { L.   Mullins },
title = {Softening of Rubber by Deformation},
journal = {Rubber Chemistry and Technology},
volume = {42},
number = {1},
pages = {339-362},
year = {1969},
}

@article {Harwood66,
author = {Harwood, J. A. C. and Payne, A. R.},
title = {Stress softening in natural rubber vulcanizates. Part IV. Unfilled vulcanizates},
journal = {Journal of Applied Polymer Science},
volume = {10},
number = {8},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
pages = {1203--1211},
year = {1966},
}


@article{Mullins49,
author = { L.   Mullins },
title = {Permanent Set in Vulcanized Rubber},
journal = {Rubber Chemistry and Technology},
volume = {22},
number = {4},
pages = {1036-1044},
year = {1949},
doi = {10.5254/1.3543010},
URL = { 
        http://dx.doi.org/10.5254/1.3543010  
},
}

@article{Blanchard52,
author = {Blanchard, A. F. and Parkinson, D.},
title = {Breakage of Carbon-Rubber Networks by Applied Stress},
journal = {Industrial \& Engineering Chemistry},
volume = {44},
number = {4},
pages = {799-812},
year = {1952},
doi = {10.1021/ie50508a034},

URL = { 
        http://dx.doi.org/10.1021/ie50508a034
},
}

@article{Houwink55,
author = { R.   Houwink },
title = {Slipping of Molecules during the Deformation of Reinforced Rubber},
journal = {Rubber Chemistry and Technology},
volume = {29},
number = {3},
pages = {888-893},
year = {1955},
doi = {10.5254/1.3542602},
}

@article {Kraus66,
author = {Kraus, G. and Childers, C. W. and Rollmann, K. W.},
title = {Stress softening in carbon black-reinforced vulcanizates. Strain rate and temperature effects},
journal = {Journal of Applied Polymer Science},
volume = {10},
number = {2},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
issn = {1097-4628},
url = {http://dx.doi.org/10.1002/app.1966.070100205},
doi = {10.1002/app.1966.070100205},
pages = {229--244},
year = {1966},
}

@article{Hanson05,
title = "Stress softening experiments in silica-filled polydimethylsiloxane provide insight into a mechanism for the Mullins effect ",
journal = "Polymer ",
volume = "46",
number = "24",
pages = "10989 - 10995",
year = "2005",
note = "",
issn = "0032-3861",
doi = "http://dx.doi.org/10.1016/j.polymer.2005.09.039",
author = "David E. Hanson and Marilyn Hawley and Robert Houlton and Kiran Chitanvis and Philip Rae and E. Bruce Orler and Debra A. Wrobleski",
}

@article {Fukahori05,
author = {Fukahori, Yoshihide},
title = {New progress in the theory and model of carbon black reinforcement of elastomers},
journal = {Journal of Applied Polymer Science},
volume = {95},
number = {1},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
issn = {1097-4628},
doi = {10.1002/app.20802},
pages = {60--67},
keywords = {carbon black, reinforcement, elastomers, interface model, crazing},
year = {2005},
}

@article{Haut89,
  title={The effects of orientation and location on the strength of dorsal rat skin in high and low speed tensile failure experiments},
  author={Haut, RC},
  journal={Journal of biomechanical engineering},
  volume={111},
  number={2},
  pages={136--140},
  year={1989},
  publisher={American Society of Mechanical Engineers}
}

@article{Dombi93,
title = "Correlation of High-Speed Tensile Strength with Collagen Content in Control and Lathyritic Rat Skin",
journal = "Journal of Surgical Research",
volume = "54",
number = "1",
pages = "21 - 28",
year = "1993",
note = "",
issn = "0022-4804",
doi = "http://dx.doi.org/10.1006/jsre.1993.1004",
url = "http://www.sciencedirect.com/science/article/pii/S0022480483710048",
author = "George W. Dombi and Roger C. Haut and Walter G. Sullivan",

}

@book{swaim90,
  title={Small animal wound management.},
  author={Swaim, Steven F and Henderson, Ralph A and Pidgeon, Rhoda S and others},
  year={1990},
  publisher={Lea \& Febiger}
}

@article{Annaidh12,
title = "Characterization of the anisotropic mechanical properties of excised human skin ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "5",
number = "1",
pages = "139 - 148",
year = "2012",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2011.08.016",
url = "http://www.sciencedirect.com/science/article/pii/S1751616111002219",
author = "Aisling Ní Annaidh and Karine Bruyère and Michel Destrade and Michael D. Gilchrist and Mélanie Otténio",
} 

@article{Munoz08,
title = "An experimental study of the mouse skin behaviour: Damage and inelastic aspects ",
journal = "Journal of Biomechanics ",
volume = "41",
number = "1",
pages = "93 - 99",
year = "2008",
note = "",
issn = "0021-9290",
doi = "http://doi.org/10.1016/j.jbiomech.2007.07.013",
url = "http://www.sciencedirect.com/science/article/pii/S002192900700320X",
author = "M.J. Muñoz and J.A. Bea and J.F. Rodríguez and I. Ochoa and J. Grasa and A. Pérez del Palomar and P. Zaragoza and R. Osta and M. Doblaré",
}

@article{Kang11,
title = "Ratchetting of porcine skin under uniaxial cyclic loading ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "4",
number = "3",
pages = "498 - 506",
year = "2011",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2010.12.015",
url = "http://www.sciencedirect.com/science/article/pii/S1751616110001906",
author = "Guozheng Kang and Xinfeng Wu",
}


@book{Berardesca95,
  title={Bioengineering of the skin: methods and instrumentation},
  author={Berardesca, Enzo and Elsner, Peter and Wilhelm, Klaus-Peter and Maibach, Howard I},
  volume={3},
  year={1995},
  publisher={CRC Press}
}

@article {Zhou10,
	author = {Zhou, B. and Xu, F. and Chen, C. Q. and Lu, T. J.},
	title = {Strain rate sensitivity of skin tissue under thermomechanical loading},
	volume = {368},
	number = {1912},
	pages = {679--690},
	year = {2010},
	doi = {10.1098/rsta.2009.0238},
	publisher = {The Royal Society},
	issn = {1364-503X},
	URL = {http://rsta.royalsocietypublishing.org/content/368/1912/679},
	eprint = {http://rsta.royalsocietypublishing.org/content/368/1912/679.full.pdf},
	journal = {Philosophical Transactions of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

@article{lanir79,
  title={The rheological behavior of the skin: experimental results and a structural model.},
  author={Lanir, Y},
  journal={Biorheology},
  volume={16},
  number={3},
  pages={191},
  year={1979}
}

@article{Ottenio15,
title = "Strain rate and anisotropy effects on the tensile failure characteristics of human skin ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "41",
number = "",
pages = "241 - 250",
year = "2015",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2014.10.006",
url = "http://www.sciencedirect.com/science/article/pii/S1751616114003282",
author = "Mélanie Ottenio and Doris Tran and Aisling Ní Annaidh and Michael D. Gilchrist and Karine Bruyère",
}

@article{Tong76,
title = "The stress-strain relationship for the skin",
journal = "Journal of Biomechanics",
volume = "9",
number = "10",
pages = "649 - 657",
year = "1976",
note = "",
issn = "0021-9290",
doi = "http://dx.doi.org/10.1016/0021-9290(76)90107-X",
url = "http://www.sciencedirect.com/science/article/pii/002192907690107X",
author = "Pin Tong and Yuang-Cheng Fung",
}

@article{Danielson73,
  title={Human skin as an elastic membrane},
  author={Danielson, DA},
  journal={Journal of Biomechanics},
  volume={6},
  number={5},
  pages={539--546},
  year={1973},
  publisher={Elsevier}
}

@article{North78,
  title={Volume compressibility of human abdominal skin},
  author={North, James F and Gibson, Francis},
  journal={Journal of biomechanics},
  volume={11},
  number={4},
  pages={203207--205},
  year={1978},
  publisher={Elsevier}
}

@ARTICLE{Pena11,
author={Pena, E.},
title={Prediction of the softening and damage effects with permanent set in fibrous biological materials},
journal={Journal of the Mechanics and Physics of Solids},
year={2011},
volume={59},
number={9},
pages={1808-1822},
doi={10.1016/j.jmps.2011.05.013},
note={cited By 26},
document_type={Article},
source={Scopus},
}

@Article{Peña10,
author="Pe{\~{n}}a, Estefania
and Calvo, B.
and Mart{\'i}nez, M. A.
and Martins, P.
and Mascarenhas, T.
and Jorge, R. M. N.
and Ferreira, A.
and Doblar{\'e}, M.",
title="Experimental study and constitutive modeling of the viscoelastic mechanical properties of the human prolapsed vaginal tissue",
journal="Biomechanics and Modeling in Mechanobiology",
year="2010",
volume="9",
number="1",
pages="35--44",
issn="1617-7940",
doi="10.1007/s10237-009-0157-2",
url="http://dx.doi.org/10.1007/s10237-009-0157-2"
}

@Article{Ehret07,
author="Ehret, Alexander E.
and Itskov, Mikhail",
title="A polyconvex hyperelastic model for fiber-reinforced materials in application to soft tissues",
journal="Journal of Materials Science",
year="2007",
volume="42",
number="21",
pages="8853--8863",
issn="1573-4803",
doi="10.1007/s10853-007-1812-6",
url="http://dx.doi.org/10.1007/s10853-007-1812-6"
}

@article{Zhu16,
title = "Logarithmic rate based elasto-viscoplastic cyclic constitutive model for soft biological tissues ",
journal = "Journal of the Mechanical Behavior of Biomedical Materials ",
volume = "61",
number = "",
pages = "397 - 409",
year = "2016",
note = "",
issn = "1751-6161",
doi = "http://doi.org/10.1016/j.jmbbm.2016.03.014",
url = "http://www.sciencedirect.com/science/article/pii/S1751616116300340",
author = "Yilin Zhu and Guozheng Kang and Chao Yu and Leong Hien Poh",
}

@ARTICLE{Humphrey87,
author={Humphrey, J.D. and Yin, F.C.},
title={A new constitutive formulation for characterizing the mechanical behavior of soft tissues.},
journal={Biophysical Journal},
year={1987},
volume={52},
number={4},
pages={563-570},
note={cited By 66},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0023428314&partnerID=40&md5=87b13645541151e194b58a3a56fef4ea},
document_type={Article},
source={Scopus},
}

@Article{,
author="Rajagopal, K. R.
and Srinivasa, A. R.",
title="An implicit three-dimensional model for describing the inelastic response of solids undergoing finite deformation",
journal="Zeitschrift f{\"u}r angewandte Mathematik und Physik",
year="2016",
volume="67",
number="4",
pages="86",
doi="10.1007/s00033-016-0671-x",
url="http://dx.doi.org/10.1007/s00033-016-0671-x"
}


@article{Tonge13,
title = "Full-field bulge test for planar anisotropic tissues: Part \{II\} – A thin shell method for determining material parameters and comparison of two distributed fiber modeling approaches ",
journal = "Acta Biomaterialia ",
volume = "9",
number = "4",
pages = "5926 - 5942",
year = "2013",
note = "",
issn = "1742-7061",
doi = "http://doi.org/10.1016/j.actbio.2012.11.034",
url = "http://www.sciencedirect.com/science/article/pii/S1742706112005843",
author = "Theresa K. Tonge and Liming M. Voo and Thao D. Nguyen",
}


@Article{Carew00,
author="Carew, E. O.
and Barber, J. E.
and Vesely, I.",
title="Role of Preconditioning and Recovery Time in Repeated Testing of Aortic Valve Tissues: Validation Through Quasilinear Viscoelastic Theory",
journal="Annals of Biomedical Engineering",
year="2000",
volume="28",
number="9",
pages="1093--1100",
issn="1573-9686",
doi="10.1114/1.1310221",
url="http://dx.doi.org/10.1114/1.1310221"
}

@ARTICLE{Giles07,
author={Giles, J.M. and Black, A.E. and Bischoff, J.E.},
title={Anomalous rate dependence of the preconditioned response of soft tissue during load controlled deformation},
journal={Journal of Biomechanics},
year={2007},
volume={40},
number={4},
pages={777-785},
doi={10.1016/j.jbiomech.2006.03.017},
note={cited By 26},
document_type={Article},
source={Scopus},
}

@article{Schriefl15,
title = "Selective enzymatic removal of elastin and collagen from human abdominal aortas: Uniaxial mechanical response and constitutive modeling ",
journal = "Acta Biomaterialia ",
volume = "17",
number = "",
pages = "125 - 136",
year = "2015",
note = "",
issn = "1742-7061",
doi = "http://doi.org/10.1016/j.actbio.2015.01.003",
url = "http://www.sciencedirect.com/science/article/pii/S1742706115000045",
author = "Andreas J. Schriefl and Thomas Schmidt and Daniel Balzani and Gerhard Sommer and Gerhard A. Holzapfel",
}

@article{Peña09,
title = "On the Mullins effect and hysteresis of fibered biological materials: A comparison between continuous and discontinuous damage models ",
journal = "International Journal of Solids and Structures ",
volume = "46",
number = "7–8",
pages = "1727 - 1735",
year = "2009",
note = "",
issn = "0020-7683",
doi = "http://doi.org/10.1016/j.ijsolstr.2008.12.015",
url = "http://www.sciencedirect.com/science/article/pii/S0020768308005179",
author = "Estefanía Peña and Juan A. Peña and Manuel Doblaré",
}


@article{MEIJER99,
author = { R.   MEIJER  and  L. F. A.   DOUVEN  and  C. W. J.   OOMENS },
title = {Characterisation of Anisotropic and Non-linear Behaviour of Human Skin In Vivo},
journal = {Computer Methods in Biomechanics and Biomedical Engineering},
volume = {2},
number = {1},
pages = {13-27},
year = {1999},
doi = {10.1080/10255849908907975},
    note ={PMID: 11264815},
}

@article{Sasso08,
title = "Characterization of hyperelastic rubber-like materials by biaxial and uniaxial stretching tests based on optical methods ",
journal = "Polymer Testing ",
volume = "27",
number = "8",
pages = "995 - 1004",
year = "2008",
note = "",
issn = "0142-9418",
doi = "https://doi.org/10.1016/j.polymertesting.2008.09.001",
url = "http://www.sciencedirect.com/science/article/pii/S0142941808001529",
author = "M. Sasso and G. Palmieri and G. Chiappini and D. Amodio",
}

@article{lanir74,
  title={Two-dimensional mechanical properties of rabbit skin—II. Experimental results},
  author={Lanir, Y and Fung, YC},
  journal={Journal of biomechanics},
  volume={7},
  number={2},
  pages={171IN9175--174182},
  year={1974},
  publisher={Elsevier}
}

@Article{Sacks00,
author="Sacks, Michael S.",
title="Biaxial Mechanical Evaluation of Planar Biological Materials",
journal="Journal of elasticity and the physical science of solids",
year="2000",
volume="61",
number="1",
pages="199",
issn="1573-2681",
doi="10.1023/A:1010917028671",
url="http://dx.doi.org/10.1023/A:1010917028671"
}

@article{lokshin09,
  title={Viscoelasticity and preconditioning of rat skin under uniaxial stretch: microstructural constitutive characterization},
  author={Lokshin, Olga and Lanir, Yoram},
  journal={Journal of biomechanical engineering},
  volume={131},
  number={3},
  pages={031009},
  year={2009},
  publisher={American Society of Mechanical Engineers}
}

@article {Rivlin51,
	author = {Rivlin, R. S. and Saunders, D. W.},
	title = {Large Elastic Deformations of Isotropic Materials. VII. Experiments on the Deformation of Rubber},
	volume = {243},
	number = {865},
	pages = {251--288},
	year = {1951},
	doi = {10.1098/rsta.1951.0004},
	publisher = {The Royal Society},
	issn = {0080-4614},
	URL = {http://rsta.royalsocietypublishing.org/content/243/865/251},
	eprint = {http://rsta.royalsocietypublishing.org/content/243/865/251.full.pdf},
	journal = {Philosophical Transactions of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

@article{obata70,
  title={Mechanical properties of natural rubber vulcanizates in finite deformation},
  author={Obata, Yutaka and Kawabata, Sueo and Kawai, Hiromichi},
  journal={Journal of Polymer Science Part A-2: Polymer Physics},
  volume={8},
  number={6},
  pages={903--919},
  year={1970},
  publisher={Wiley Online Library}
}

@inproceedings{korochkina05,
  title={Choosing constitutive models for elastomers used in printing processes},
  author={Korochkina, TV and Claypole, TC and Gethin, DT},
  booktitle={CONSTITUTIVE MODELS FOR RUBBER-PROCEEDINGS-},
  volume={4},
  pages={431},
  year={2005},
  organization={Balkema}
}

@Article{Wineman15,
author="Wineman, Alan
and Rajagopal, K. R.",
title="A constitutive theory for multi-functional fiber reinforced composites",
journal="Acta Mechanica",
year="2015",
volume="226",
number="8",
pages="2671--2679",
issn="1619-6937",
doi="10.1007/s00707-015-1345-z",
url="http://dx.doi.org/10.1007/s00707-015-1345-z"
}

@article{ayoub16,
  title={Heart valve biomechanics and underlying mechanobiology},
  author={Ayoub, Salma and Ferrari, Giovanni and Gorman, Robert C and Gorman, Joseph H and Schoen, Frederick J and Sacks, Michael S},
  journal={Comprehensive Physiology},
  year={2016},
  publisher={Wiley Online Library}
}

@article{frisen69,
  title={Rheological analysis of soft collagenous tissue: Part I: Theoretical considerations},
  author={Frisen, M and M{\"a}gi, M and Sonnerup, L and Viidik, A},
  journal={Journal of Biomechanics},
  volume={2},
  number={1},
  pages={13--20},
  year={1969},
  publisher={Elsevier}
}

@article{frisen1969b,
  title={Rheological analysis of soft collagenous tissue: Part II: Experimental evaluations and verifications},
  author={Frisen, M and M{\"a}gi, M and Sonnerup, L and Viidik, A},
  journal={Journal of biomechanics},
  volume={2},
  number={1},
  pages={21--28},
  year={1969},
  publisher={Elsevier}
}

@article{sacks03,
  title={Incorporation of experimentally-derived fiber orientation into a structural constitutive model for planar collagenous tissues},
  author={Sacks, Michael S and others},
  journal={TRANSACTIONS-AMERICAN SOCIETY OF MECHANICAL ENGINEERS JOURNAL OF BIOMECHANICAL ENGINEERING},
  volume={125},
  number={2},
  pages={280--287},
  year={2003},
  publisher={AMERICAN SOCIETY MECHANICAL ENGINEERS}
}

@article{sellaro07,
  title={Effects of collagen fiber orientation on the response of biologically derived soft tissue biomaterials to cyclic loading},
  author={Sellaro, Tiffany L and Hildebrand, Daniel and Lu, Qijin and Vyavahare, Naren and Scott, Michael and Sacks, Michael S},
  journal={Journal of Biomedical Materials Research Part A},
  volume={80},
  number={1},
  pages={194--205},
  year={2007},
  publisher={Wiley Online Library}
}

@Article{Freed16,
author="Freed, Alan D.
and Rajagopal, K. R.",
title="A promising approach for modeling biological fibers",
journal="Acta Mechanica",
year="2016",
month="Jun",
day="01",
volume="227",
number="6",
pages="1609--1619",
}


@article{Zhang16,
title = "A meso-scale layer-specific structural constitutive model of the mitral heart valve leaflets",
journal = "Acta Biomaterialia",
volume = "32",
number = "Supplement C",
pages = "238 - 255",
year = "2016",
issn = "1742-7061",
doi = "https://doi.org/10.1016/j.actbio.2015.12.001",
url = "http://www.sciencedirect.com/science/article/pii/S1742706115302397",
author = "Will Zhang and Salma Ayoub and Jun Liao and Michael S. Sacks",
}

@ARTICLE{Pena11,
author={Pena, E.},
title={Prediction of the softening and damage effects with permanent set in fibrous biological materials},
journal={Journal of the Mechanics and Physics of Solids},
year={2011},
volume={59},
number={9},
pages={1808-1822},
doi={10.1016/j.jmps.2011.05.013},
note={cited By 26},
document_type={Article},
source={Scopus},
}

@Article{Pena10,
author="Pe{\~{n}}a, Estefania
and Calvo, B.
and Mart{\'i}nez, M. A.
and Martins, P.
and Mascarenhas, T.
and Jorge, R. M. N.
and Ferreira, A.
and Doblar{\'e}, M.",
title="Experimental study and constitutive modeling of the viscoelastic mechanical properties of the human prolapsed vaginal tissue",
journal="Biomechanics and Modeling in Mechanobiology",
year="2010",
volume="9",
number="1",
pages="35--44",
issn="1617-7940",
doi="10.1007/s10237-009-0157-2",
url="http://dx.doi.org/10.1007/s10237-009-0157-2"
}


@article{Pena09,
title = "On the Mullins effect and hysteresis of fibered biological materials: A comparison between continuous and discontinuous damage models ",
journal = "International Journal of Solids and Structures ",
volume = "46",
number = "7–8",
pages = "1727 - 1735",
year = "2009",
note = "",
issn = "0020-7683",
doi = "http://doi.org/10.1016/j.ijsolstr.2008.12.015",
url = "http://www.sciencedirect.com/science/article/pii/S0020768308005179",
author = "Estefanía Peña and Juan A. Peña and Manuel Doblaré",
}


@article{LIAO99,
title = "A failure model for ligaments",
journal = "Journal of Biomechanics",
volume = "32",
number = "2",
pages = "183 - 188",
year = "1999",
issn = "0021-9290",
doi = "https://doi.org/10.1016/S0021-9290(98)00169-9",
url = "http://www.sciencedirect.com/science/article/pii/S0021929098001699",
author = "Hongyan Liao and Stephen M. Belkoff",
keywords = "Failure, Structural model, Collagen, Ligament"
}

@article{HILL12,
title = "A theoretical and non-destructive experimental approach for direct inclusion of measured collagen orientation and recruitment into mechanical models of the artery wall",
journal = "Journal of Biomechanics",
volume = "45",
number = "5",
pages = "762 - 771",
year = "2012",
note = "Special Issue on Cardiovascular Solid Mechanics",
issn = "0021-9290",
doi = "https://doi.org/10.1016/j.jbiomech.2011.11.016",
url = "http://www.sciencedirect.com/science/article/pii/S0021929011006981",
author = "Michael R. Hill and Xinjie Duan and Gregory A. Gibson and Simon Watkins and Anne M. Robertson",
keywords = "Collagen fiber, Collagen recruitment, Orientation distribution function, Uniaxial testing, Multi-photon microscopy"
}

@article{Benias18,
  title={Structure and Distribution of an Unrecognized Interstitium in Human Tissues},
  author={Benias, Petros C and Wells, Rebecca G and Sackey-Aboagye, Bridget and Klavan, Heather and Reidy, Jason and Buonocore, Darren and Miranda, Markus and Kornacki, Susan and Wayne, Michael and Carr-Locke, David L and others},
  journal={Scientific reports},
  volume={8},
  number={1},
  pages={4947},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{Mullin48,
author = { L.   Mullins },
title = {Effect of Stretching on the Properties of Rubber},
journal = {Rubber Chemistry and Technology},
volume = {21},
number = {2},
pages = {281-300},
year = {1948},
doi = {10.5254/1.3546914},
URL = { https://doi.org/10.5254/1.3546914},
eprint = { https://doi.org/10.5254/1.3546914}
}


@article{XU08,
title = "Biothermomechanics of skin tissues",
journal = "Journal of the Mechanics and Physics of Solids",
volume = "56",
number = "5",
pages = "1852 - 1884",
year = "2008",
issn = "0022-5096",
doi = "https://doi.org/10.1016/j.jmps.2007.11.011",
url = "http://www.sciencedirect.com/science/article/pii/S002250960700227X",
author = "F. Xu and T.J. Lu and K.A. Seffen",
keywords = "Skin tissue, Biothermomechanics, Analytical model, Numerical method, Thermal"
}

@article{Afsar18,
title = "Inelastic Response of Skin under Uniaxial Cyclic Mechanical Loading-Multinetwork Model Comparison with Experiments ",
journal = "International Journal of Engineering Science",
volume = "",
number = "",
pages = "",
year = "Under Review",
note = "",
issn = "",
doi = "",
url = "",
author = "N. Afsar Kazerooni and A.R. Srinivasa and J.C. Criscione"
}

@article{Zhu14,
title = "A finite viscoelastic–plastic model for describing the uniaxial ratchetting of soft biological tissues",
journal = "Journal of Biomechanics",
volume = "47",
number = "5",
pages = "996 - 1003",
year = "2014",
issn = "0021-9290",
doi = "https://doi.org/10.1016/j.jbiomech.2014.01.004",
url = "http://www.sciencedirect.com/science/article/pii/S0021929014000177",
author = "Yilin Zhu and Guozheng Kang and Qianhua Kan and Chao Yu",
keywords = "Soft biological tissues, Constitutive model, Anisotropy, Ratchetting, Time-dependence"
}

@article{LOKSHIN091,
title = "Micro and macro rheology of planar tissues",
journal = "Biomaterials",
volume = "30",
number = "17",
pages = "3118 - 3127",
year = "2009",
issn = "0142-9612",
doi = "https://doi.org/10.1016/j.biomaterials.2009.02.039",
url = "http://www.sciencedirect.com/science/article/pii/S0142961209002312",
author = "Olga Lokshin and Yoram Lanir",
}

@InProceedings{Nava04,
author="Nava, Alessandro
and Mazza, Edoardo
and Haefner, Oliver
and Bajka, Michael",
editor="Cotin, St{\'e}phane
and Metaxas, Dimitris",
title="Experimental Observation and Modelling of Preconditioning in Soft Biological Tissues",
booktitle="Medical Simulation",
year="2004",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="1--8",
isbn="978-3-540-25968-8"
}

@article{Avis00,
author = {N. J. Avis},
title = {Virtual environment technologies},
journal = {Minimally Invasive Therapy \& Allied Technologies},
volume = {9},
number = {5},
pages = {333-339},
year  = {2000},
publisher = {Taylor & Francis},
doi = {10.3109/13645700009061455},
}

@article{Satava99,
  title={Virtual reality in medicine},
  author={Satava, Richard M and others},
  journal={Bmj},
  volume={319},
  number={7220},
  pages={1305},
  year={1999},
  publisher={British Medical Journal Publishing Group}
}


@Article{Eshel01,
author="Eshel, H.
and Lanir, Y.",
title="Effects of Strain Level and Proteoglycan Depletion on Preconditioning and Viscoelastic Responses of Rat Dorsal Skin",
journal="Annals of Biomedical Engineering",
year="2001",
month="Feb",
day="01",
volume="29",
number="2",
pages="164--172",
issn="1573-9686",
}

@book{srinivasa09,
  title={Inelasticity of materials: an engineering approach and a practical guide},
  author={Srinivasa, Arun R and Srinivasan, Sivakumar M},
  volume={80},
  year={2009},
  publisher={World Scientific Publishing Company}
}




